Domain-specific or Uncertainty-aware models: Does it really make a difference for biomedical text classification?

The success of pretrained language models (PLMs) across a spate of use-cases has led to significant investment from the NLP community towards building domain-specific foundational models. On the other hand, in mission critical settings such as biomedical applications, other aspects also factor in-chief of which is a model's ability to produce reasonable estimates of its own uncertainty. In the present study, we discuss these two desiderata through the lens of how they shape the entropy of a model's output probability distribution. We find that domain specificity and uncertainty awareness can often be successfully combined, but the exact task at hand weighs in much more strongly.

==> Figures/beeswarm.tex <==
\begin{figure}
    \centering
    \includegraphics[scale=0.4, clip, trim=0 0.71cm 0 0]{Figures/entropy_unce.pdf}
    \caption{ENTROPY}
    \label{fig:enter-label}
\end{figure}

==> Figures/unc_shap.tex <==
\begin{figure}
    \centering % <-- added
\includegraphics[scale=0.46]{Figures/uncertain-shap.pdf}
\caption{Relative Importance via SHAP}
\label{fig:rel-imp}
\end{figure}

==> Tables/TRESULTS.tex <==
\begin{table*}[]
    \centering
    \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{lrrrrr}
\toprule
 & val acc & test acc & brier & CE & ECE \\
setup &  &  &  &  &  \\
\midrule
bert-dnn-MEDABS-1e-5-4 & 0.604224 & 0.609765 & 0.110706 & NaN & NaN \\
%bert-dnn-MORFITT-5e-5-15 & 0.545662 & 0.505208 & 0.068204 & NaN & NaN \\
bert-dropconnect-MEDABS-1e-6-15 & 0.608380 & 0.611034 & 0.111407 & 0.491631 & 0.200000 \\
%bert-dropconnect-MORFITT-1e-5-15 & 0.581213 & 0.551471 & 0.052879 & 0.458761 & 0.083333 \\
bert-mc dropout-MEDABS-5e-6-6 & 0.603994 & 0.607456 & 0.111033 & 0.443875 & 0.200000 \\
%bert-mc dropout-MORFITT-5e-5-15 & 0.562296 & 0.527880 & 0.064514 & 0.493468 & 0.083333 \\
bert-variational inf-MEDABS-5e-6-7 & 0.606648 & 0.611034 & 0.113977 & 0.494574 & 0.200000 \\
%bert-variational inf-MORFITT-5e-5-11 & 0.544684 & 0.509191 & 0.067832 & 0.495893 & 0.083333 \\
\midrule
biobert-dnn-MEDABS-1e-5-3 & 0.615420 & 0.619114 & 0.108597 & NaN & NaN \\
%biobert-dnn-MORFITT-5e-5-14 & 0.595564 & 0.562194 & 0.060541 & NaN & NaN \\
biobert-dropconnect-MEDABS-5e-6-7 & 0.622922 & 0.616343 & 0.109960 & 0.493102 & 0.200000 \\
%biobert-dropconnect-MORFITT-5e-5-13 & 0.603718 & 0.562500 & 0.062730 & 0.497197 & 0.083333 \\
biobert-mc dropout-MEDABS-1e-4-3 & 0.616805 & 0.620960 & 0.107158 & 0.461222 & 0.200000 \\
%biobert-mc dropout-MORFITT-5e-5-12 & 0.597847 & 0.551471 & 0.059172 & 0.476484 & 0.083333 \\
biobert-variational inf-MEDABS-1e-5-5 & 0.622576 & 0.636196 & 0.106333 & 0.494888 & 0.200000 \\
%biobert-variational inf-MORFITT-1e-5-15 & 0.606654 & 0.570466 & 0.054141 & 0.493224 & 0.083333 \\
\midrule
camembert-dnn-MORFITT-5e-5-11 & 0.639922 & 0.594363 & 0.049274 & NaN & NaN \\
camembert-dropconnect-MORFITT-5e-5-15 & 0.657208 & 0.621630 & 0.055225 & 0.496077 & 0.083333 \\
camembert-mc dropout-MORFITT-5e-5-14 & 0.648076 & 0.603248 & 0.050423 & 0.427325 & 0.083333 \\
camembert-variational inf-MORFITT-5e-5-14 & 0.658839 & 0.613051 & 0.055818 & 0.496133 & 0.083333 \\
\midrule
biocamembert-dnn-MORFITT-5e-5-10 & 0.649380 & 0.600184 & 0.049257 & NaN & NaN \\
biocamembert-dropconnect-MORFITT-5e-5-7 & 0.670907 & 0.629289 & 0.045881 & 0.411362 & 0.083333 \\
biocamembert-mc dropout-MORFITT-5e-5-13 & 0.650033 & 0.606311 & 0.048457 & 0.394636 & 0.083333 \\
biocamembert-variational inf-MORFITT-5e-5-6 & 0.673190 & 0.632966 & 0.047249 & 0.476454 & 0.083333 \\
\midrule
camembert-dropconnect 	PXCORPUS 	5e-6 	14 &0.888889 	&0.874055\\
camembert-mcdropout 	PXCORPUS 	1e-5 	14&0.905724 &	0.879093\\
camembert-dnn 	PXCORPUS 	1e-5 	14 & 0.904040 	&0.880772\\
camembert-variationalinf 	PXCORPUS 	1e-5 	10 & 0.932660 	&0.905961\\
\midrule
biocamembert-variational inf-PXCORPUS-1e-5-12 & 0.914141 &  	0.881612\\
biocamembert-dropconnect 	1e-5 	15& 0.909091 &	0.883291\\
biocamembert-dnn 	PXCORPUS 	1e-5 	15& 0.917508& 	0.902603\\
biocamembert-mcdropout 	PXCORPUS 	1e-5 	14 & 0.925926 	&0.912678\\


\bottomrule
\end{tabular}}
    \caption{results from grid search}
    \label{tab:my_label}
\end{table*}

==> Tables/comparison.tex <==
  \begin{table}[]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|c|cccc|}
        \hline
         & \multicolumn{4}{c|}{\texttt{MORFITT}} \\
        \textbf{Model} &  val-F1($\uparrow$) & test-F1($\uparrow$) & Brier-score($\downarrow$) & ECE($\downarrow$)\\
        \hline
        vanilla-DNN & 33.36$\pm$3.03& 32.93$\pm$2.23 &0.0743$\pm$0.0027 &0.2470$\pm$0.0123\\
        MCDropout & 36.69$\pm$4.02 & 35.63$\pm$3.16 & 0.0750$\pm$0.0022&0.2500$\pm$0.0258\\
        DROPConnect & 36.30$\pm$3.82 & 35.24$\pm$2.86 & 0.0738$\pm$0.0030& 0.2392$\pm$0.0325\\
        Variational-Inf & 37.28$\pm$3.76 & 35.86$\pm$2.83 & 0.0743$\pm$0.0028&0.2411$\pm$0.0285\\
        \hline
        & \multicolumn{4}{c|}{\texttt{MEDABS}} \\
        \textbf{Model} &  val-F1($\uparrow$) & test-F1($\uparrow$) & Brier-score($\downarrow$) & ECE($\downarrow$)\\
        \hline
        vanilla-DNN & 55.19$\pm$0.69 & 55.77$\pm$0.35 & 0.1458$\pm$0.0014 & 0.2281$\pm$0.0061 \\
        MCDropout & 55.04$\pm$0.98 & 55.63$\pm$0.70 & 0.1483$\pm$0.0026 & 0.2256$\pm$0.0152\\
        DROPConnect & 55.22$\pm$1.05 & 55.56$\pm$0.34 & 0.1479$\pm$0.0025 & 0.2222$\pm$0.0135\\
        Variational-Inf & 54.73$\pm$1.01 & 55.37$\pm$0.91 & 0.1499$\pm$0.0037 & 0.2251$\pm$0.0142\\
        \hline
    \end{tabular}}
    \caption{Model Comparison for Performance (macro-F1) and Uncertainty :  epochs=15, fine-tuning($\checkmark$), hyperparam-search($\times$)}
    \label{tab:models_stat}
\end{table}

==> Tables/main-results-typestting.tex <==
\begin{table*}[!th]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{rcc ccccccccc}
    \toprule
       & \multicolumn{2}{c}{\multirow{2}{*}{Model}} &  \multicolumn{2}{c}{Classification}& &  \multicolumn{6}{c}{Uncertainty}\\
        \cmidrule{4-5} \cmidrule{7-12}
            &&& Macro-F1($\uparrow$) & Accuracy($\uparrow$)& & BS($\downarrow$) & ECE($\downarrow$) & SCE($\downarrow$)  & NLL($\downarrow$) & Coverage\%($\uparrow$) & Entropy($\downarrow$) \\
    \midrule
        \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{MedABS}}} & 
        $-\mathcal{D}$ & $-\mathcal{U}$ & 0.602246 & 0.608495&&\underline{0.551441} &	\textbf{0.134095} &	\underline{0.066295} &	1.331350 &	\underline{0.896353}&1.560235\\
         & $+\mathcal{D}$ & $-\mathcal{U}$ & \underline{0.611547}  & 0.608610&& 0.571310 &	 0.180296 &	 0.077107 &	\underline{1.310785} &	\textbf{0.912512}	&\textbf{1.548926}\\
         & \rowcolor{gray!20} $-\mathcal{D}$ & $+\mathcal{U}$ & 0.606620 &\underline{0.611034}&&0.557037   &	0.145812   &	0.069479   &	1.325999 &	0.855494  &1.557213\\
         & \rowcolor{gray!20}$+\mathcal{D}$ & $+\mathcal{U}$ &\textbf{0.632524}&\textbf{0.628116}&&\textbf{0.523878}& 	\underline{0.140859} &	\textbf{0.062842} &	\textbf{1.291286} &	0.856994  &\underline{1.550856}  \\
         \midrule
         %=============================================================================
         \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{MedNLI}}} & $-\mathcal{D}$ & $-\mathcal{U}$ & 0.733705& 0.733240&& 0.402373& 	\textbf{0.115560} &	\textbf{0.077374} &	0.828362 	&\textbf{0.928504} &	1.020356\\
         & $+\mathcal{D}$ & $-\mathcal{U}$ & \underline{0.803858} &\underline{0.804301} &&\underline{0.360875} 	&0.147122 &	0.099788 	&\underline{0.766016} &	0.863338 &	\underline{0.995832}\\
         & \rowcolor{gray!20} $-\mathcal{D}$ & $+\mathcal{U}$ & 0.754503 &0.754805&	&0.435817 &	0.202691 	&0.136461 &	0.790006& 	0.807079 &	\textbf{0.988143} \\
         & \rowcolor{gray!20} $+\mathcal{D}$ & $+\mathcal{U}$& \textbf{0.804982}& \textbf{0.805907}&& \textbf{0.313292}& \underline{0.120978} &	\underline{0.082146} &	\textbf{0.744658} &	\underline{0.877637} &	0.997812\\
         \midrule
         %=============================================================================
         \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{SMOKING}}} & 
         $-\mathcal{D}$ & $-\mathcal{U}$ & \underline{0.250739} & 0.384615&&\underline{0.669931} &	\underline{0.170088} &	\underline{0.132612} &	1.473753 &	0.612179&1.588659\\
         & $+\mathcal{D}$ & $-\mathcal{U}$ &  0.228513& 0.461538&& 0.802114 &	 0.340216 &	 0.161939 &	\underline{1.421092} &	\textbf{0.682692}&\textbf{1.546859}\\
         & \rowcolor{gray!20} $-\mathcal{D}$ & $+\mathcal{U}$ & 0.233007&\underline{0.483974}&&\textbf{0.620675} &	\textbf{0.127112} &	\textbf{0.109565} &	1.421468 &	\underline{0.647436}&1.578952\\
         & \rowcolor{gray!20} $+\mathcal{D}$ & $+\mathcal{U}$ &\textbf{0.270123}&\textbf{0.487179}&& 0.763660 &	 0.273658 &	 0.154944 	&\textbf{1.411110} &	 0.541667  &\underline{1.551109}  \\
         \midrule
         %=============================================================================
         \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{PxSLU}}} & 
         $-\mathcal{D}$ & $-\mathcal{U}$ & 0.319693 & 0.880772&&0.533842 &	0.467537 &	0.276416 &	1.261665 &	\textbf{0.997481}&1.380891\\
         & $+\mathcal{D}$ & $-\mathcal{U}$ & \underline{0.381850} & \textbf{0.902603}&&0.479364 &	0.415783 &	0.274239 	&1.221917 &	 \underline{0.973132}&1.378235\\
         & \rowcolor{gray!20} $-\mathcal{D}$ & $+\mathcal{U}$ &0.353205 &0.874055&&\underline{0.365078} &	\underline{0.316629} &	\underline{0.212358} 	&\underline{1.145101}& 	{0.962217}  &\underline{1.368281}\\
         & \rowcolor{gray!20} $+\mathcal{D}$ & $+\mathcal{U}$ &\textbf{0.420834}&\underline{0.883291}&&\textbf{0.227683} &	\textbf{0.159425} &	\textbf{0.137527} &	\textbf{1.001403} &	 {0.962217}   &\textbf{1.335407}\\
         \midrule
         %=============================================================================
         \multirow{4}{*}{\parbox[t]{2mm}{\rotatebox[origin=c]{90}{MedMCQA}}} & 
         $-\mathcal{D}$ & $-\mathcal{U}$ & 0.280453& 0.629689&&0.725581 	&0.352222 &	0.171180 &	1.566691& 	0.983387&1.608586\\
         & $+\mathcal{D}$ & $-\mathcal{U}$ & 0.294744 & \underline{0.656484}&&\underline{0.696034} 	& 0.354713 &	\textbf{0.152432} &	\underline{1.546633} 	& 0.981243&\underline{1.607683}\\
         & \rowcolor{gray!20} $-\mathcal{D}$ & $+\mathcal{U}$ & \underline{0.308781}&	0.579850&&0.725009 &	\underline{0.303931} &	0.157625 &	1.567476   	&\textbf{0.988210}&1.608650  \\
         & \rowcolor{gray!20} $+\mathcal{D}$ & $+\mathcal{U}$ &\textbf{0.346549}&\textbf{0.696141}&&\textbf{0.673225} 	&\textbf{0.274169}& 	\underline{0.152654}   &	\textbf{1.524824} &	 \underline{0.987138}&\textbf{1.603390}\\
         \midrule
         %=============================================================================
         \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{MORFITT}}} & 
         $-\mathcal{D}$ & $-\mathcal{U}$ & 0.499836 & 0.594363&&\underline{0.591286} &	\textbf{0.060664} &	0.039075& 	2.171540 &	\underline{0.877757}&2.466179\\
         & $+\mathcal{D}$ & $-\mathcal{U}$ & \underline{0.535068} & \underline{0.616728}&& 0.597271 	& 0.195975 &	\textbf{0.034757} 	&\underline{2.055853} 	& 0.837929& \underline{2.446618}\\
         & \rowcolor{gray!20} $-\mathcal{D}$ & $+\mathcal{U}$ &0.503970 &0.580576&&\textbf{0.587825} &	\underline{0.073795}   &	\underline{0.040320}   &	2.180531   &	\textbf{0.883272}&2.467595  \\
         & \rowcolor{gray!20} $+\mathcal{D}$ & $+\mathcal{U}$ &\textbf{0.555584}&\textbf{0.625919}&& 0.623643   &	 0.254945   &	 0.043031   &	\textbf{2.015742}& 	 0.754289  &\textbf{2.436898}\\
         \bottomrule
    \end{tabular}
    }
    \caption{Comparison for text classification performance and uncertainty-awareness. We report the mean of 3 seed runs for all the metrics. We denote best score with \textbf{bold} and second best with \underline{underline}. % Here, $-\mathcal{D}~+\mathcal{U}$ denotes {DropConnect} as it was on average the best ranked model across all the best configurations.  
    }
    \label{tab:finalcomparisontable}
\end{table*}

==> Tables/main-results.tex <==
\begin{table*}[!th]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{rc ccccccccc}
    \toprule
       & \multirow{2}{*}{Model} &  \multicolumn{2}{c}{Classification}& &  \multicolumn{6}{c}{Uncertainty}\\
        \cmidrule{3-4} \cmidrule{6-11}
            && Macro-F1($\uparrow$) & Accuracy($\uparrow$)& & BS($\downarrow$) & ECE($\downarrow$) & SCE($\downarrow$)  & NLL($\downarrow$) & Coverage\%($\uparrow$) & Entropy($\downarrow$) \\
    \midrule
        \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{MedABS}}} & 
        DNN & 0.602246 & 0.608495&&\underline{0.551441} &	\textbf{0.134095} &	\underline{0.066295} &	1.331350 &	\underline{0.896353}&1.560235\\
         & bioDNN & \underline{0.611547}  & 0.608610&& 0.571310 &	 0.180296 &	 0.077107 &	\underline{1.310785} &	\textbf{0.912512}	&\textbf{1.548926}\\
         & \rowcolor{gray!20} BNN & 0.606620 &\underline{0.611034}&&0.557037   &	0.145812   &	0.069479   &	1.325999 &	0.855494  &1.557213\\
         & \rowcolor{gray!20}bioBNN &\textbf{0.632524}&\textbf{0.628116}&&\textbf{0.523878}& 	\underline{0.140859} &	\textbf{0.062842} &	\textbf{1.291286} &	0.856994  &\underline{1.550856}  \\
         \midrule
         %=============================================================================
         \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{MedNLI}}} & DNN & 0.733705& 0.733240&& 0.402373& 	\textbf{0.115560} &	\textbf{0.077374} &	0.828362 	&\textbf{0.928504} &	1.020356\\
         & bioDNN & \underline{0.803858} &\underline{0.804301} &&\underline{0.360875} 	&0.147122 &	0.099788 	&\underline{0.766016} &	0.863338 &	\underline{0.995832}\\
         & \rowcolor{gray!20} BNN & 0.754503 &0.754805&	&0.435817 &	0.202691 	&0.136461 &	0.790006& 	0.807079 &	\textbf{0.988143} \\
         & \rowcolor{gray!20} bioBNN& \textbf{0.804982}& \textbf{0.805907}&& \textbf{0.313292}& \underline{0.120978} &	\underline{0.082146} &	\textbf{0.744658} &	\underline{0.877637} &	0.997812\\
         \midrule
         %=============================================================================
         \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{SMOKING}}} & 
         DNN & \underline{0.250739} & 0.384615&&\underline{0.669931} &	\underline{0.170088} &	\underline{0.132612} &	1.473753 &	0.612179&1.588659\\
         & bioDNN &  0.228513& 0.461538&& 0.802114 &	 0.340216 &	 0.161939 &	\underline{1.421092} &	\textbf{0.682692}&\textbf{1.546859}\\
         & \rowcolor{gray!20} BNN & 0.233007&\underline{0.483974}&&\textbf{0.620675} &	\textbf{0.127112} &	\textbf{0.109565} &	1.421468 &	\underline{0.647436}&1.578952\\
         & \rowcolor{gray!20} bioBNN &\textbf{0.270123}&\textbf{0.487179}&& 0.763660 &	 0.273658 &	 0.154944 	&\textbf{1.411110} &	 0.541667  &\underline{1.551109}  \\
         \midrule
         %=============================================================================
         \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{PxSLU}}} & 
         DNN & 0.319693 & 0.880772&&0.533842 &	0.467537 &	0.276416 &	1.261665 &	\textbf{0.997481}&1.380891\\
         & bioDNN & \underline{0.381850} & \textbf{0.902603}&&0.479364 &	0.415783 &	0.274239 	&1.221917 &	 \underline{0.973132}&1.378235\\
         & \rowcolor{gray!20} BNN &0.353205 &0.874055&&\underline{0.365078} &	\underline{0.316629} &	\underline{0.212358} 	&\underline{1.145101}& 	{0.962217}  &\underline{1.368281}\\
         & \rowcolor{gray!20} bioBNN &\textbf{0.420834}&\underline{0.883291}&&\textbf{0.227683} &	\textbf{0.159425} &	\textbf{0.137527} &	\textbf{1.001403} &	 {0.962217}   &\textbf{1.335407}\\
         \midrule
         %=============================================================================
         \multirow{4}{*}{\parbox[t]{2mm}{\rotatebox[origin=c]{90}{MedMCQA}}} & 
         DNN & 0.280453& 0.629689&&0.725581 	&0.352222 &	0.171180 &	1.566691& 	0.983387&1.608586\\
         & bioDNN & 0.294744 & \underline{0.656484}&&\underline{0.696034} 	& 0.354713 &	\textbf{0.152432} &	\underline{1.546633} 	& 0.981243&\underline{1.607683}\\
         & \rowcolor{gray!20} BNN & \underline{0.308781}&	0.579850&&0.725009 &	\underline{0.303931} &	0.157625 &	1.567476   	&\textbf{0.988210}&1.608650  \\
         & \rowcolor{gray!20} bioBNN &\textbf{0.346549}&\textbf{0.696141}&&\textbf{0.673225} 	&\textbf{0.274169}& 	\underline{0.152654}   &	\textbf{1.524824} &	 \underline{0.987138}&\textbf{1.603390}\\
         \midrule
         %=============================================================================
         \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{MORFITT}}} & 
         DNN & 0.499836 & 0.594363&&\underline{0.591286} &	\textbf{0.060664} &	0.039075& 	2.171540 &	\underline{0.877757}&2.466179\\
         & bioDNN & \underline{0.535068} & \underline{0.616728}&& 0.597271 	& 0.195975 &	\textbf{0.034757} 	&\underline{2.055853} 	& 0.837929& \underline{2.446618}\\
         & \rowcolor{gray!20} BNN &0.503970 &0.580576&&\textbf{0.587825} &	\underline{0.073795}   &	\underline{0.040320}   &	2.180531   &	\textbf{0.883272}&2.467595  \\
         & \rowcolor{gray!20} bioBNN &\textbf{0.555584}&\textbf{0.625919}&& 0.623643   &	 0.254945   &	 0.043031   &	\textbf{2.015742}& 	 0.754289  &\textbf{2.436898}\\
         \bottomrule
    \end{tabular}
    }
    \caption{Comparison for text classification performance and uncertainty-awareness. We report the mean of 3 seed runs for all the metrics. We denote best score with \textbf{bold} and second best with \underline{underline}. Here, BNN denotes {DropConnect} as it was on average the best ranked model across all the best configurations.  }
    \label{tab:finalcomparisontable}
\end{table*}

==> Tables/perfcomparsion.tex <==
\begin{table*}[!th]
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{l|ccccrr}
        \toprule
        dataset-config & valF1 & testF1 & valACC & testACC & Rank($\mathbb{D}$)&Wins($\mathbb{D}$)\\
        \midrule
        biocamembert 	dnn 	PXCORPUS 	1e-5 	15 &	0.508540 &	0.381850 &	0.917508 &	0.902603 &2&+1\\
        biocamembert 	dropconnect 	PXCORPUS 	1e-5 	15& 	0.552240 	&0.420834 &	0.909091 &	0.883291* &1&+1\\
        biocamembert 	mcdropout 	PXCORPUS 	1e-5 	14& 	0.480407 &	0.374772* &	0.925926 	&0.912678 &3&+1\\
        biocamembert 	variationalinf 	PXCORPUS 	1e-5 	12& 	0.598706 &	0.367639* &	\cellcolor{red!25}0.914141 	&\cellcolor{red!25}0.881612* &4&+1\\
        \hdashline
        camembert 	dnn 	PXCORPUS 	1e-5 	14& 	0.419015 &	0.319693 &	0.904040 &	0.880772 &4\\
        camembert 	dropconnect 	PXCORPUS 	5e-6 	14& 	0.444511& 	0.353205 &	0.888889 &	0.874055* &1\\
        camembert 	mcdropout 	PXCORPUS 	1e-5 	14& 	0.427300 &	0.324014 &	0.905724 &	0.879093* &2	\\
        camembert 	variationalinf 	PXCORPUS 	1e-5 	10& 	0.381643 &	0.320360 &	0.932660 &	0.905961 &3\\
        \midrule
        %===========================================================
        biocamembert 	dnn 	MEDMCQA 	5e-6 	15& 	0.292463& 	0.294744 &	0.658120 &	0.656484 &3&+1\\
        biocamembert 	mcdropout 	MEDMCQA 	1e-5 	14 &	0.351649& 	0.346549 &	0.688034 &	0.696141 &1&+1\\
        biocamembert 	dropconnect 	MEDMCQA 	5e-6 	14& 	0.315419 &	0.319079 &	0.602564 &	\cellcolor{red!25}0.600214* &2&+1\\
        biocamembert 	variationalinf 	MEDMCQA 	1e-6 	15& 	0.256144 &	0.261096* &	0.504274 	&0.475884* &4&+1\\
        \hdashline
        camembert 	dnn 	MEDMCQA 	5e-6 	11 	&0.275823 &	0.280453& 	0.621795 &	0.629689&3 	\\
        camembert 	dropconnect 	MEDMCQA 	1e-6 	15& 	0.336988& 	0.308781 	&0.603632 &	0.579850*&1 \\
        camembert 	mcdropout 	MEDMCQA 	5e-6 	11 &	0.299136 &	0.289972 &	0.600427 &	0.604502*&2 \\
        camembert 	variationalinf 	MEDMCQA 	1e-6 	15& 	0.227966 &	0.235716* &	0.443376 &	0.475348* &4\\
        \midrule
        %===========================================================
        biobert 	dnn 	SMOKING 	1e-4 	15 	&0.288649 &	\cellcolor{red!25}0.228513 &	0.570000 &	0.461538 	&4&\\
        biobert 	dropconnect 	SMOKING 	5e-5 	13 &	0.307604 &	0.270123 &	\cellcolor{red!25}0.513333 &	0.487179 	&2&+1\\
        biobert 	mcdropout 	SMOKING 	5e-5 	13& 	\cellcolor{red!25}0.261372& 	0.271852 &	\cellcolor{red!25}0.486667 &	0.474359&1&+1\\
        biobert 	variationalinf 	SMOKING 	5e-5 	13& 	\cellcolor{red!25}0.255114& \cellcolor{red!25}	0.228792 &	0.453333 &	0.403846*&3\\
        \hdashline
        bert 	dnn 	SMOKING 	5e-5 	9 &	0.286698 &	0.250739 &	0.393333 &	0.384615&2&+1\\
        bert 	dropconnect 	SMOKING 	1e-5 	14 &	0.293240 &	0.233007* 	&0.533333 &	0.483974&4\\
        bert 	mcdropout 	SMOKING 	5e-5 	14 &	0.274621 &	0.267451 &	0.496667 	&0.483974&1\\
        bert 	variationalinf 	SMOKING 	5e-6 	10 &	0.293946 &	0.245189* &	0.440000 &	0.365385*&3&+1\\
        \midrule
        %===========================================================
        biobert 	dnn 	MEDABS 	5e-5 	5& 	0.610897 	&0.611547 	&0.608610 	&0.608610&4&+1\\
        biobert 	dropconnect 	MEDABS 	5e-5 	3 &	0.625038 &	0.632524 &	0.621191 &	0.628116&1&+1\\
        biobert 	mcdropout 	MEDABS 	1e-4 	3 	&0.616999 &	0.621431& 	0.616805 	&0.620960 	&3&+1\\
        biobert 	variationalinf 	MEDABS 	1e-4 	4 &	0.623211 	&0.624282 &	0.620383 &	0.620845 	&2&+1\\        
        \hdashline
        
        bert 	dnn 	MEDABS 	5e-6 	6 	&0.598042 &	0.602246 	&0.604224 &	0.608495&4\\
        bert 	dropconnect 	MEDABS 	1e-6 	15 &	0.603601 	&0.606620 &	0.608380 &	0.611034&2\\
        bert 	mcdropout 	MEDABS 	5e-5 	3 &	0.597338 &	0.603760 	&0.597415 &	0.602031*&3\\
        bert 	variationalinf 	MEDABS 	1e-5 	4 &	0.605711 &	0.612985 &	0.605032 &	0.611380&1\\
        \midrule
        %===========================================================
        biocamembert 	dnn 	MORFITT 	5e-5 	15 &	0.562259 &	0.535068 &	0.649380 &	0.616728&2&+1\\
        biocamembert 	dropconnect 	MORFITT 	5e-5 	11& 	0.582032 &	0.555584 &	0.651011 &	0.625919&1&+1\\
        biocamembert 	mcdropout 	MORFITT 	5e-5 	15 &	0.561026& 	0.525568* 	&\cellcolor{red!25}0.643183 &	0.611520*&4&+1\\
        biocamembert 	variationalinf 	MORFITT 	1e-5 	14& 	0.597141 &	\cellcolor{red!25}0.528093* &	0.668297 &	\cellcolor{red!25}0.608456*&3\\
        \hdashline
        camembert 	dnn 	MORFITT 	5e-5 	11& 	0.548426 &	0.499836 &	0.639922 &	0.594363 &4	\\
        camembert 	dropconnect 	MORFITT 	5e-5 	6 	&0.573211 	&0.503970& 	0.649706 &	0.580576*&3\\
        camembert 	mcdropout 	MORFITT 	5e-5 	14& 	0.560971 &	0.511796 &	0.648076 &	0.603248&2\\
        camembert 	variationalinf 	MORFITT 	5e-5 	10& 	0.576202 &	0.535038 &	0.653947 &	0.614890 &1&+1\\
        \midrule
        %===========================================================
        bert 	dnn 	MEDNLI 	5e-6 	10 &	0.764749 &	0.733705 	&0.765114 	&0.733240  \\
bert dropconnect 	MEDNLI 	1e-5 	15& 	0.771405 &	0.754503 &	0.772999 &	0.754805   \\
bert mcdropout 	MEDNLI 	1e-5 	8 &	0.757966 &	0.729950 &	0.759140 &	0.730427 	\\
bert variationalinf 	MEDNLI 	1e-5 	14& 	0.749048 &	0.720887 &	0.750777 &	0.721050   \\
biobert 	dnn 	MEDNLI 	1e-5 	12& 	0.803858 &	0.787442 &	0.804301 &	0.787389 	\\
biobert dropconnect 	MEDNLI 	5e-6 	11& 	0.820472 &	0.804982 	&0.821983 	&0.805907 \\
biobert mcdropout 	MEDNLI 	1e-5 	15& 	0.814237 &	0.803008 &	0.814815 &	0.802860   \\
biobert variationalinf 	MEDNLI 	5e-6 	13& 	0.769356 &	0.759109 &	0.771565 &	0.760431  \\
        %===========================================================
        %\rowcolor{gray!45}
        %& val-mae 	&test-mae &	val-rmse &	test-rmse \\
        
        
        %biobert 	dnn regressor 	BIOSSES 	5e-4 	12& 	0.900200 	&1.184433& 	1.114300 	&1.387067 &2&+1\\
        %biobert 	dc regressor 	BIOSSES 	1e-6 	98 &	\cellcolor{red!25}1.412633 	&\cellcolor{red!25}1.627133 &	\cellcolor{red!25}1.650567 &\cellcolor{red!25}	1.931433&4\\
        %biobert 	mcd regressor 	BIOSSES 	1e-5 	13 &	\cellcolor{red!25}0.879900 &	\cellcolor{red!25}1.191433 &	\cellcolor{red!25}1.088433 &	\cellcolor{red!25}1.402167&3&\\
        %biobert 	vi regressor 	BIOSSES 	5e-4 	16 &	1.191400 &	1.161567 &	1.420900 	&1.419900 &1&+1\\
        %\hdashline
        %bert 	dnn regressor 	BIOSSES 	5e-4 	11 &	1.084600 &	1.385167 &	1.331533 &	1.619300&4 \\
        %bert 	dc regressor 	BIOSSES 	1e-6 	84& 	1.132667 &	1.375867 &	1.356667 	&1.620067  &3&+1\\
        %bert 	mcd regressor 	BIOSSES 	5e-4 	4 	&0.792567 &	1.146767 	&1.034533 &	1.318533&1 &+1\\
        %bert 	vi regressor 	BIOSSES 	5e-6 	21 &	1.240867 &	1.279133 &	1.523233 &	1.484567&2 \\
        %============================================================
         \bottomrule
    \end{tabular}
    }
    \caption{New Performance Table; * denotes unexpected score compared to DNN counterpart}
    \label{tab:newperf}
\end{table*}

==> Tables/redo/main-results-typesetting-new.tex <==
\begin{table*}[!h]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{rcc ccccccccc}
    \toprule
       & \multicolumn{2}{c}{\multirow{2}{*}{Model}} &  \multicolumn{2}{c}{Classification}& &  \multicolumn{6}{c}{Uncertainty}\\
        \cmidrule{4-5} \cmidrule{7-12}
            &&& Macro-F1($\uparrow$) & Accuracy($\uparrow$)& & BS($\downarrow$) & ECE($\downarrow$) & SCE($\downarrow$)  & NLL($\downarrow$) & Coverage\%($\uparrow$) & Entropy($\downarrow$) \\
    \midrule
     %=============================================================================
     & 
          $-\mathcal{D}$ & $-\mathcal{U}$ &60.3633$\pm$\tiny{0.003}&60.9765$\pm$\tiny{0.002}&&0.5535$\pm$\tiny{0.008}&0.1387$\pm$\tiny{0.016}&0.0683$\pm$\tiny{0.004}&1.3261$\pm$\tiny{0.001}&0.8976$\pm$\tiny{0.013}&1.5579$\pm$\tiny{0.002}\\
&  $+\mathcal{D}$ & $-\mathcal{U}$ &\underline{60.9855}$\pm$\tiny{0.004}&61.1842$\pm$\tiny{0.003}&&0.5518$\pm$\tiny{0.002}&\textbf{0.1342}$\pm$\tiny{0.007}&\underline{0.0674}$\pm$\tiny{0.003}&\underline{1.3192}$\pm$\tiny{0.002}&\textbf{0.9611}$\pm$\tiny{0.003}&\underline{1.5556}$\pm$\tiny{0.001}\\
%&  mc dropout&60.5487$\pm$\tiny{0.012}&60.3878$\pm$\tiny{0.012}&&0.5515$\pm$\tiny{0.013}&0.1197$\pm$\tiny{0.019}&0.063$\pm$\tiny{0.005}&1.3298$\pm$\tiny{0.006}&0.9635$\pm$\tiny{0.004}&1.5598$\pm$\tiny{0.001}\\
%&  variational inf&61.2727$\pm$\tiny{0.016}&61.1842$\pm$\tiny{0.015}&&0.5417$\pm$\tiny{0.018}&0.1197$\pm$\tiny{0.013}&0.0615$\pm$\tiny{0.012}&1.3202$\pm$\tiny{0.011}&0.9602$\pm$\tiny{0.002}&1.5579$\pm$\tiny{0.001}\\
\rowcolor{gray!20} &$-\mathcal{D}$ & $+\mathcal{U}$&60.8077$\pm$\tiny{0.013}&\underline{61.3343}$\pm$\tiny{0.01}&&\underline{0.5499}$\pm$\tiny{0.014}&0.1448$\pm$\tiny{0.005}&0.0695$\pm$\tiny{0.001}&1.3201$\pm$\tiny{0.014}&0.9193$\pm$\tiny{0.005}&1.5561$\pm$\tiny{0.003}\\

\rowcolor{gray!20}\parbox[t]{2mm}{\multirow{-4}{*}{\rotatebox[origin=c]{90}{MedABS}}} 
&$+\mathcal{D}$ & $+\mathcal{U}$&\textbf{62.5642}$\pm$\tiny{0.009}&\textbf{62.1018}$\pm$\tiny{0.01}&&\textbf{0.5243}$\pm$\tiny{0.015}&\underline{0.1381}$\pm$\tiny{0.016}&\textbf{0.0624}$\pm$\tiny{0.007}&\textbf{1.2962}$\pm$\tiny{0.007}&\underline{0.9597}$\pm$\tiny{0.008}&\textbf{1.5523}$\pm$\tiny{0.002}\\
\midrule
%&bio  mc dropout&62.0348$\pm$\tiny{0.007}&61.9806$\pm$\tiny{0.006}&&0.5314$\pm$\tiny{0.023}&0.1054$\pm$\tiny{0.021}&0.0615$\pm$\tiny{0.007}&1.3231$\pm$\tiny{0.023}&0.9619$\pm$\tiny{0.012}&1.5609$\pm$\tiny{0.006}\\
%&bio  variational inf&62.0845$\pm$\tiny{0.012}&61.7498$\pm$\tiny{0.013}&&0.5328$\pm$\tiny{0.041}&0.1526$\pm$\tiny{0.058}&0.0647$\pm$\tiny{0.023}&1.2942$\pm$\tiny{0.008}&0.9426$\pm$\tiny{0.031}&1.5496$\pm$\tiny{0.009}\\
         %=============================================================================
          & 
          $-\mathcal{D}$ & $-\mathcal{U}$ &73.8951$\pm$\tiny{0.013}&73.8397$\pm$\tiny{0.015}&&0.3976$\pm$\tiny{0.006}&\textbf{0.1278}$\pm$\tiny{0.02}&\textbf{0.0846}$\pm$\tiny{0.012}&0.8177$\pm$\tiny{0.015}&\textbf{0.9119}$\pm$\tiny{0.008}&1.0156$\pm$\tiny{0.008} \\
& $+\mathcal{D}$ & $-\mathcal{U}$ &74.8161$\pm$\tiny{0.019}&74.8711$\pm$\tiny{0.018}&&0.4242$\pm$\tiny{0.021}&0.185$\pm$\tiny{0.007}&0.1259$\pm$\tiny{0.005}&0.7945$\pm$\tiny{0.014}&0.8509$\pm$\tiny{0.007}&\underline{0.9941}$\pm$\tiny{0.002} \\
%& mc dropout&73.0181$\pm$\tiny{0.018}&73.0661$\pm$\tiny{0.017}&&0.4083$\pm$\tiny{0.021}&0.1221$\pm$\tiny{0.008}&0.0862$\pm$\tiny{0.005}&0.8261$\pm$\tiny{0.014}&0.9372$\pm$\tiny{0.002}&1.0174$\pm$\tiny{0.002} \\
%& variational inf&72.1177$\pm$\tiny{0.033}&72.1519$\pm$\tiny{0.034}&&0.4489$\pm$\tiny{0.016}&0.1814$\pm$\tiny{0.018}&0.1251$\pm$\tiny{0.012}&0.8195$\pm$\tiny{0.03}&0.8645$\pm$\tiny{0.043}&1.0016$\pm$\tiny{0.013} \\
\rowcolor{gray!20}& $-\mathcal{D}$ & $+\mathcal{U}$&\underline{77.172}$\pm$\tiny{0.041}&\underline{77.2386}$\pm$\tiny{0.039}&&\underline{0.3783}$\pm$\tiny{0.05}&0.1579$\pm$\tiny{0.009}&0.107$\pm$\tiny{0.007}&\underline{0.7736}$\pm$\tiny{0.039}&0.857$\pm$\tiny{0.015}&0.9952$\pm$\tiny{0.008} \\
\rowcolor{gray!20}\parbox[t]{2mm}{\multirow{-4}{*}{\rotatebox[origin=c]{90}{MedNLI}}}&
$+\mathcal{D}$ & $+\mathcal{U}$&\textbf{79.9945}$\pm$\tiny{0.037}&\textbf{80.0047}$\pm$\tiny{0.037}&&\textbf{0.3375}$\pm$\tiny{0.045}&\underline{0.1392}$\pm$\tiny{0.005}&\underline{0.0956}$\pm$\tiny{0.002}&\textbf{0.7486}$\pm$\tiny{0.041}&\underline{0.8872}$\pm$\tiny{0.011}&\textbf{0.9924}$\pm$\tiny{0.011} \\ \midrule
%&bio mc dropout&80.3488$\pm$\tiny{0.028}&80.3329$\pm$\tiny{0.028}&&0.3406$\pm$\tiny{0.028}&0.1435$\pm$\tiny{0.01}&0.0973$\pm$\tiny{0.007}&0.7485$\pm$\tiny{0.03}&0.872$\pm$\tiny{0.015}&0.9912$\pm$\tiny{0.01} \\
%&bio variational inf&76.032$\pm$\tiny{0.041}&76.1603$\pm$\tiny{0.04}&&0.3619$\pm$\tiny{0.052}&0.0987$\pm$\tiny{0.009}&0.0751$\pm$\tiny{0.011}&0.7982$\pm$\tiny{0.042}&0.9398$\pm$\tiny{0.013}&1.0145$\pm$\tiny{0.01} \\
 
%=============================================================================
        
          & 
          $-\mathcal{D}$ & $-\mathcal{U}$ &\textbf{27.1141}$\pm$\tiny{0.041}&45.8333$\pm$\tiny{0.142}&&0.7724$\pm$\tiny{0.054}&0.2961$\pm$\tiny{0.057}&0.154$\pm$\tiny{0.012}&1.4298$\pm$\tiny{0.106}&\underline{0.7724}$\pm$\tiny{0.163}&\underline{1.5536}$\pm$\tiny{0.028}\\
&  $+\mathcal{D}$ & $-\mathcal{U}$ &25.7924$\pm$\tiny{0.041}&46.7949$\pm$\tiny{0.039}&&\textbf{0.6407}$\pm$\tiny{0.035}&\textbf{0.1625}$\pm$\tiny{0.043}&\textbf{0.1215}$\pm$\tiny{0.016}&1.4331$\pm$\tiny{0.035}&\textbf{0.9455}$\pm$\tiny{0.031}&1.5791$\pm$\tiny{0.01}\\
%&  mc dropout&26.9919$\pm$\tiny{0.006}&48.3974$\pm$\tiny{0.078}&&0.7043$\pm$\tiny{0.064}&0.2278$\pm$\tiny{0.035}&0.1334$\pm$\tiny{0.028}&1.4305$\pm$\tiny{0.057}&0.875$\pm$\tiny{0.058}&1.5674$\pm$\tiny{0.009}\\
%&  variational inf&22.4613$\pm$\tiny{0.014}&33.6538$\pm$\tiny{0.017}&&0.7214$\pm$\tiny{0.029}&0.1907$\pm$\tiny{0.032}&0.1522$\pm$\tiny{0.016}&1.5192$\pm$\tiny{0.021}&0.9455$\pm$\tiny{0.055}&1.5939$\pm$\tiny{0.003}\\
\rowcolor{gray!20}& $-\mathcal{D}$ & $+\mathcal{U}$&24.9822$\pm$\tiny{0.041}&\textbf{51.6026}$\pm$\tiny{0.071}&&\underline{0.6764}$\pm$\tiny{0.076}&\underline{0.2262}$\pm$\tiny{0.013}&\underline{0.1334}$\pm$\tiny{0.031}&\textbf{1.3928}$\pm$\tiny{0.068}&0.6571$\pm$\tiny{0.114}&1.5596$\pm$\tiny{0.011}\\
\parbox[t]{2mm}{\multirow{-4}{*}{\rotatebox[origin=c]{90}{SMOKING}}}\rowcolor{gray!20}&$+\mathcal{D}$ & $+\mathcal{U}$&\underline{27.0293}$\pm$\tiny{0.033}&\underline{47.1154}$\pm$\tiny{0.075}&&0.841$\pm$\tiny{0.043}&0.3441$\pm$\tiny{0.053}&0.1738$\pm$\tiny{0.007}&\underline{1.4297}$\pm$\tiny{0.06}&0.7276$\pm$\tiny{0.118}&\textbf{1.5419}$\pm$\tiny{0.02}\\ \midrule
%&bio  mc dropout&26.8859$\pm$\tiny{0.008}&47.1154$\pm$\tiny{0.019}&&0.6843$\pm$\tiny{0.07}&0.224$\pm$\tiny{0.054}&0.1294$\pm$\tiny{0.036}&1.4363$\pm$\tiny{0.012}&0.9167$\pm$\tiny{0.062}&1.5732$\pm$\tiny{0.009}\\
%&bio  variational inf&24.3715$\pm$\tiny{0.041}&41.0256$\pm$\tiny{0.087}&&0.774$\pm$\tiny{0.019}&0.2724$\pm$\tiny{0.058}&0.1672$\pm$\tiny{0.014}&1.4467$\pm$\tiny{0.061}&0.8045$\pm$\tiny{0.024}&1.5601$\pm$\tiny{0.018}\\

%=============================================================================
          & 
          $-\mathcal{D}$ & $-\mathcal{U}$&32.2541$\pm$\tiny{0.075}&\underline{88.2452}$\pm$\tiny{0.012}&&0.5743$\pm$\tiny{0.077}&0.4556$\pm$\tiny{0.094}&0.2955$\pm$\tiny{0.014}&1.2807$\pm$\tiny{0.05}&0.995$\pm$\tiny{0.004}&1.3821$\pm$\tiny{0.003}\\
& $+\mathcal{D}$ & $-\mathcal{U}$ &\underline{34.1464}$\pm$\tiny{0.026}&84.2989$\pm$\tiny{0.05}&&\underline{0.4599}$\pm$\tiny{0.088}&0.3936$\pm$\tiny{0.047}&\underline{0.2354}$\pm$\tiny{0.03}&\underline{1.2154}$\pm$\tiny{0.062}&\textbf{1.0}$\pm$\tiny{0.0}&1.3768$\pm$\tiny{0.007}\\
%& mc dropout&32.4014$\pm$\tiny{0.076}&87.9093$\pm$\tiny{0.015}&&0.5412$\pm$\tiny{0.107}&0.4905$\pm$\tiny{0.092}&0.2667$\pm$\tiny{0.028}&1.2684$\pm$\tiny{0.064}&1.0$\pm$\tiny{0.0}&1.3815$\pm$\tiny{0.004}\\
%& variational inf&31.546$\pm$\tiny{0.137}&90.3442$\pm$\tiny{0.012}&&0.3913$\pm$\tiny{0.213}&0.374$\pm$\tiny{0.201}&0.1959$\pm$\tiny{0.085}&1.1455$\pm$\tiny{0.185}&0.9966$\pm$\tiny{0.006}&1.3612$\pm$\tiny{0.034}\\
\rowcolor{gray!20}& $-\mathcal{D}$ & $+\mathcal{U}$&33.1131$\pm$\tiny{0.097}&80.1763$\pm$\tiny{0.238}&&0.5389$\pm$\tiny{0.116}&\underline{0.3929}$\pm$\tiny{0.057}&0.2867$\pm$\tiny{0.037}&1.2548$\pm$\tiny{0.06}&0.9831$\pm$\tiny{0.018}&\underline{1.38}$\pm$\tiny{0.003}\\
\rowcolor{gray!20}\parbox[t]{2mm}{\multirow{-4}{*}{\rotatebox[origin=c]{90}{PXSLU}}}&$+\mathcal{D}$ & $+\mathcal{U}$&\textbf{40.3372}$\pm$\tiny{0.07}&\textbf{89.1184}$\pm$\tiny{0.039}&&\textbf{0.2649}$\pm$\tiny{0.127}&\textbf{0.2576}$\pm$\tiny{0.105}&\textbf{0.1568}$\pm$\tiny{0.058}&\textbf{1.0539}$\pm$\tiny{0.111}&\underline{0.9997}$\pm$\tiny{0.001}&\textbf{1.3496}$\pm$\tiny{0.021}\\ \midrule
%&bio mc dropout&37.4772$\pm$\tiny{0.031}&91.2678$\pm$\tiny{0.013}&&0.5048$\pm$\tiny{0.04}&0.5048$\pm$\tiny{0.019}&0.2609$\pm$\tiny{0.014}&1.2472$\pm$\tiny{0.026}&1.0$\pm$\tiny{0.0}&1.3805$\pm$\tiny{0.002}\\
%&bio variational inf&37.3134$\pm$\tiny{0.046}&88.2452$\pm$\tiny{0.057}&&0.225$\pm$\tiny{0.111}&0.205$\pm$\tiny{0.089}&0.1255$\pm$\tiny{0.055}&1.0117$\pm$\tiny{0.109}&0.9992$\pm$\tiny{0.001}&1.34$\pm$\tiny{0.024}\\

%=============================================================================
          & 
          $-\mathcal{D}$ & $-\mathcal{U}$&28.5727$\pm$\tiny{0.03}&\textbf{63.88}$\pm$\tiny{0.055}&&0.6787$\pm$\tiny{0.1}&0.3256$\pm$\tiny{0.043}&0.1575$\pm$\tiny{0.021}&1.5347$\pm$\tiny{0.062}&0.9625$\pm$\tiny{0.033}&1.6063$\pm$\tiny{0.003}\\
& $+\mathcal{D}$ & $-\mathcal{U}$ &\textbf{32.0291}$\pm$\tiny{0.003}&\underline{63.5584}$\pm$\tiny{0.007}&&\textbf{0.4822}$\pm$\tiny{0.015}&\textbf{0.165}$\pm$\tiny{0.01}&\textbf{0.1099}$\pm$\tiny{0.0}&\textbf{1.3846}$\pm$\tiny{0.009}&0.9764$\pm$\tiny{0.007}&\textbf{1.5888}$\pm$\tiny{0.001}\\
%& mc dropout&28.3648$\pm$\tiny{0.029}&61.3612$\pm$\tiny{0.103}&&0.7533$\pm$\tiny{0.044}&0.3819$\pm$\tiny{0.084}&0.1518$\pm$\tiny{0.02}&1.5848$\pm$\tiny{0.024}&1.0$\pm$\tiny{0.0}&1.6091$\pm$\tiny{0.0}\\
%& variational inf&23.1977$\pm$\tiny{0.042}&48.5531$\pm$\tiny{0.046}&&0.7499$\pm$\tiny{0.023}&0.242$\pm$\tiny{0.033}&0.1329$\pm$\tiny{0.004}&1.5822$\pm$\tiny{0.013}&1.0$\pm$\tiny{0.0}&1.6089$\pm$\tiny{0.0}\\
\rowcolor{gray!20} & $-\mathcal{D}$ & $+\mathcal{U}$&28.1549$\pm$\tiny{0.045}&61.0932$\pm$\tiny{0.089}&&0.6859$\pm$\tiny{0.12}&0.3026$\pm$\tiny{0.009}&0.1582$\pm$\tiny{0.01}&1.5388$\pm$\tiny{0.077}&\underline{0.9775}$\pm$\tiny{0.02}&1.6064$\pm$\tiny{0.004}\\
\rowcolor{gray!20}\parbox[t]{2mm}{\multirow{-4}{*}{\rotatebox[origin=c]{90}{MedMCQA}}}&$+\mathcal{D}$ & $+\mathcal{U}$&\underline{29.7558}$\pm$\tiny{0.07}&60.343$\pm$\tiny{0.103}&&\underline{0.6687}$\pm$\tiny{0.17}&\underline{0.2973}$\pm$\tiny{0.069}&\underline{0.1278}$\pm$\tiny{0.018}&\underline{1.5216}$\pm$\tiny{0.122}&\textbf{0.9893}$\pm$\tiny{0.019}&\underline{1.6025}$\pm$\tiny{0.012}\\
\midrule
%&bio mc dropout&32.0019$\pm$\tiny{0.013}&70.5788$\pm$\tiny{0.012}&&0.5655$\pm$\tiny{0.096}&0.3481$\pm$\tiny{0.06}&0.1551$\pm$\tiny{0.025}&1.4663$\pm$\tiny{0.068}&0.9962$\pm$\tiny{0.006}&1.602$\pm$\tiny{0.006}\\
%&bio variational inf&27.5691$\pm$\tiny{0.012}&52.3044$\pm$\tiny{0.024}&&0.7294$\pm$\tiny{0.021}&0.2559$\pm$\tiny{0.018}&0.1266$\pm$\tiny{0.004}&1.5701$\pm$\tiny{0.012}&1.0$\pm$\tiny{0.0}&1.6084$\pm$\tiny{0.001}\\
%=============================================================================
          & 
          $-\mathcal{D}$ & $-\mathcal{U}$&49.7506$\pm$\tiny{0.009}&59.038$\pm$\tiny{0.012}&&0.6499$\pm$\tiny{0.022}&0.2323$\pm$\tiny{0.021}&\underline{0.0398}$\pm$\tiny{0.005}&2.0748$\pm$\tiny{0.015}&0.796$\pm$\tiny{0.045}&2.4454$\pm$\tiny{0.003}\\
& $+\mathcal{D}$ & $-\mathcal{U}$ &\underline{55.4551}$\pm$\tiny{0.01}&\underline{62.5306}$\pm$\tiny{0.008}&&\underline{0.6134}$\pm$\tiny{0.003}&\underline{0.2243}$\pm$\tiny{0.003}&0.0425$\pm$\tiny{0.001}&\underline{2.0332}$\pm$\tiny{0.006}&\textbf{0.8775}$\pm$\tiny{0.014}&\underline{2.4411}$\pm$\tiny{0.001}\\
%& mc dropout&51.2184$\pm$\tiny{0.02}&60.386$\pm$\tiny{0.018}&&0.5877$\pm$\tiny{0.009}&0.0934$\pm$\tiny{0.021}&0.0308$\pm$\tiny{0.002}&2.1249$\pm$\tiny{0.028}&0.9427$\pm$\tiny{0.006}&2.4589$\pm$\tiny{0.004}\\
%& variational inf&53.6771$\pm$\tiny{0.017}&61.4583$\pm$\tiny{0.025}&&0.6024$\pm$\tiny{0.049}&0.1905$\pm$\tiny{0.074}&0.0392$\pm$\tiny{0.009}&2.0513$\pm$\tiny{0.026}&0.8725$\pm$\tiny{0.06}&2.4452$\pm$\tiny{0.007}\\

\rowcolor{gray!20}& $-\mathcal{D}$ & $+\mathcal{U}$&53.4963$\pm$\tiny{0.019}&61.8015$\pm$\tiny{0.014}&&\textbf{0.6081}$\pm$\tiny{0.017}&\textbf{0.2098}$\pm$\tiny{0.014}&\textbf{0.0363}$\pm$\tiny{0.002}&2.0538$\pm$\tiny{0.015}&0.8334$\pm$\tiny{0.01}&2.4453$\pm$\tiny{0.002}\\
\rowcolor{gray!20}\parbox[t]{2mm}{\multirow{-4}{*}{\rotatebox[origin=c]{90}{MORFITT}}}&$+\mathcal{D}$ & $+\mathcal{U}$&\textbf{56.4418}$\pm$\tiny{0.018}&\textbf{62.9596}$\pm$\tiny{0.02}&&0.6148$\pm$\tiny{0.027}&0.2325$\pm$\tiny{0.018}&0.0433$\pm$\tiny{0.003}&\textbf{2.0251}$\pm$\tiny{0.015}&\underline{0.8667}$\pm$\tiny{0.03}&\textbf{2.4394}$\pm$\tiny{0.001}\\ 
         \bottomrule
%&bio mc dropout&52.6114$\pm$\tiny{0.008}&61.2132$\pm$\tiny{0.004}&&0.5942$\pm$\tiny{0.004}&0.1275$\pm$\tiny{0.027}&0.0332$\pm$\tiny{0.003}&2.1046$\pm$\tiny{0.021}&0.9455$\pm$\tiny{0.002}&2.4551$\pm$\tiny{0.003}\\
%&bio variational inf&53.2133$\pm$\tiny{0.01}&61.5502$\pm$\tiny{0.006}&&0.5449$\pm$\tiny{0.005}&0.0546$\pm$\tiny{0.005}&0.0324$\pm$\tiny{0.001}&2.1594$\pm$\tiny{0.008}&0.9911$\pm$\tiny{0.003}&2.4675$\pm$\tiny{0.001}\\
    \end{tabular}
    }
    \caption{Comparison for text classification performance and uncertainty-awareness. We report the mean and stdev of 10 seed runs for all the metrics. We denote best score with \textbf{bold} and second best with \underline{underline}. % Here, $-\mathcal{D}~+\mathcal{U}$ denotes {$+\mathcal{D}$ & $-\mathcal{U}$ } as it was on average the best ranked model across all the best configurations.  
    }
    \label{tab:finalcomparisontable-main}
\end{table*}


==> Tables/redo/table2article_new.tex <==
\begin{table*}[!th]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{rc ccccccccc}
    \toprule
       & \multirow{2}{*}{Model} &  \multicolumn{2}{c}{Classification}& &  \multicolumn{6}{c}{Uncertainty}\\
        \cmidrule{3-4} \cmidrule{6-11}
            && Macro-F1($\uparrow$) & Accuracy($\uparrow$)& & BS($\downarrow$) & ECE($\downarrow$) & SCE($\downarrow$)  & NLL($\downarrow$) & Coverage\%($\uparrow$) & Entropy($\downarrow$) \\
    \midrule
    
         \parbox[t]{2mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{MedABS}}} & 
         DNN &60.3633$\pm$\tiny{0.003}&60.9765$\pm$\tiny{0.002}&&0.5535$\pm$\tiny{0.008}&0.1387$\pm$\tiny{0.016}&0.0683$\pm$\tiny{0.004}&1.3261$\pm$\tiny{0.001}&0.8976$\pm$\tiny{0.013}&1.5579$\pm$\tiny{0.002}\\
&  dropconnect&60.9855$\pm$\tiny{0.004}&61.1842$\pm$\tiny{0.003}&&0.5518$\pm$\tiny{0.002}&0.1342$\pm$\tiny{0.007}&0.0674$\pm$\tiny{0.003}&1.3192$\pm$\tiny{0.002}&0.9611$\pm$\tiny{0.003}&1.5556$\pm$\tiny{0.001}\\
&  mc dropout&60.5487$\pm$\tiny{0.012}&60.3878$\pm$\tiny{0.012}&&0.5515$\pm$\tiny{0.013}&0.1197$\pm$\tiny{0.019}&0.063$\pm$\tiny{0.005}&1.3298$\pm$\tiny{0.006}&\textbf{0.9635$\pm$\tiny{0.004}}&1.5598$\pm$\tiny{0.001}\\
&  variational inf&61.2727$\pm$\tiny{0.016}&61.1842$\pm$\tiny{0.015}&&0.5417$\pm$\tiny{0.018}&0.1197$\pm$\tiny{0.013}&\textbf{0.0615$\pm$\tiny{0.012}}&1.3202$\pm$\tiny{0.011}&0.9602$\pm$\tiny{0.002}&1.5579$\pm$\tiny{0.001}\\
&bio  dnn&60.8077$\pm$\tiny{0.013}&61.3343$\pm$\tiny{0.01}&&0.5499$\pm$\tiny{0.014}&0.1448$\pm$\tiny{0.005}&0.0695$\pm$\tiny{0.001}&1.3201$\pm$\tiny{0.014}&0.9193$\pm$\tiny{0.005}&1.5561$\pm$\tiny{0.003}\\
&bio  dropconnect&\textbf{62.5642$\pm$\tiny{0.009}}&\textbf{62.1018$\pm$\tiny{0.01}}&&\textbf{0.5243$\pm$\tiny{0.015}}&0.1381$\pm$\tiny{0.016}&0.0624$\pm$\tiny{0.007}&\textbf{1.2962$\pm$\tiny{0.007}}&0.9597$\pm$\tiny{0.008}&1.5523$\pm$\tiny{0.002}\\
&bio  mc dropout&{62.0348$\pm$\tiny{0.007}}&\underline{61.9806$\pm$\tiny{0.006}}&&0.5314$\pm$\tiny{0.023}&\textbf{0.1054$\pm$\tiny{0.021}}&\textbf{0.0615$\pm$\tiny{0.007}}&1.3231$\pm$\tiny{0.023}&0.9619$\pm$\tiny{0.012}&1.5609$\pm$\tiny{0.006}\\
&bio  variational inf&\underline{62.0845$\pm$\tiny{0.012}}&61.7498$\pm$\tiny{0.013}&&0.5328$\pm$\tiny{0.041}&0.1526$\pm$\tiny{0.058}&0.0647$\pm$\tiny{0.023}&1.2942$\pm$\tiny{0.008}&0.9426$\pm$\tiny{0.031}&\textbf{1.5496$\pm$\tiny{0.009}} \\
\midrule
         %=============================================================================
         \parbox[t]{2mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{MedNLI}}} & 
         DNN &73.8951$\pm$\tiny{0.013}&73.8397$\pm$\tiny{0.015}&&0.3976$\pm$\tiny{0.006}&0.1278$\pm$\tiny{0.02}&0.0846$\pm$\tiny{0.012}&0.8177$\pm$\tiny{0.015}&0.9119$\pm$\tiny{0.008}&1.0156$\pm$\tiny{0.008} \\
& dropconnect&74.8161$\pm$\tiny{0.019}&74.8711$\pm$\tiny{0.018}&&0.4242$\pm$\tiny{0.021}&0.185$\pm$\tiny{0.007}&0.1259$\pm$\tiny{0.005}&0.7945$\pm$\tiny{0.014}&0.8509$\pm$\tiny{0.007}&0.9941$\pm$\tiny{0.002} \\
& mc dropout&73.0181$\pm$\tiny{0.018}&73.0661$\pm$\tiny{0.017}&&0.4083$\pm$\tiny{0.021}&\textbf{0.1221$\pm$\tiny{0.008}}&0.0862$\pm$\tiny{0.005}&0.8261$\pm$\tiny{0.014}&0.9372$\pm$\tiny{0.002}&1.0174$\pm$\tiny{0.002} \\
& variational inf&72.1177$\pm$\tiny{0.033}&72.1519$\pm$\tiny{0.034}&&0.4489$\pm$\tiny{0.016}&0.1814$\pm$\tiny{0.018}&0.1251$\pm$\tiny{0.012}&0.8195$\pm$\tiny{0.03}&0.8645$\pm$\tiny{0.043}&1.0016$\pm$\tiny{0.013} \\
&bio dnn&77.172$\pm$\tiny{0.041}&77.2386$\pm$\tiny{0.039}&&0.3783$\pm$\tiny{0.05}&0.1579$\pm$\tiny{0.009}&0.107$\pm$\tiny{0.007}&0.7736$\pm$\tiny{0.039}&0.857$\pm$\tiny{0.015}&0.9952$\pm$\tiny{0.008} \\
&bio dropconnect&\underline{79.9945$\pm$\tiny{0.037}}&\underline{80.0047$\pm$\tiny{0.037}}&&\textbf{0.3375$\pm$\tiny{0.045}}&0.1392$\pm$\tiny{0.005}&0.0956$\pm$\tiny{0.002}&0.7486$\pm$\tiny{0.041}&0.8872$\pm$\tiny{0.011}&0.9924$\pm$\tiny{0.011} \\
&bio mc dropout&\textbf{80.3488$\pm$\tiny{0.028}}&\textbf{80.3329$\pm$\tiny{0.028}}&&0.3406$\pm$\tiny{0.028}&0.1435$\pm$\tiny{0.01}&0.0973$\pm$\tiny{0.007}&\textbf{0.7485$\pm$\tiny{0.03}}&0.872$\pm$\tiny{0.015}&\textbf{0.9912$\pm$\tiny{0.01}} \\
&bio variational inf&76.032$\pm$\tiny{0.041}&76.1603$\pm$\tiny{0.04}&&0.3619$\pm$\tiny{0.052}&0.0987$\pm$\tiny{0.009}&\textbf{0.0751$\pm$\tiny{0.011}}&0.7982$\pm$\tiny{0.042}&\textbf{0.9398$\pm$\tiny{0.013}}&1.0145$\pm$\tiny{0.01} \\
 \midrule
%=============================================================================
        
         \parbox[t]{2mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{SMOKING}}} & 
         DNN &\textbf{27.1141$\pm$\tiny{0.041}}&45.8333$\pm$\tiny{0.142}&&0.7724$\pm$\tiny{0.054}&0.2961$\pm$\tiny{0.057}&0.154$\pm$\tiny{0.012}&1.4298$\pm$\tiny{0.106}&0.7724$\pm$\tiny{0.163}&1.5536$\pm$\tiny{0.028}\\
&  dropconnect&25.7924$\pm$\tiny{0.041}&46.7949$\pm$\tiny{0.039}&&\textbf{0.6407$\pm$\tiny{0.035}}&\textbf{0.1625$\pm$\tiny{0.043}}&\textbf{0.1215$\pm$\tiny{0.016}}&1.4331$\pm$\tiny{0.035}&\textbf{0.9455$\pm$\tiny{0.031}}&1.5791$\pm$\tiny{0.01}\\
&  mc dropout&26.9919$\pm$\tiny{0.006}&\underline{48.3974$\pm$\tiny{0.078}}&&0.7043$\pm$\tiny{0.064}&0.2278$\pm$\tiny{0.035}&0.1334$\pm$\tiny{0.028}&1.4305$\pm$\tiny{0.057}&0.875$\pm$\tiny{0.058}&1.5674$\pm$\tiny{0.009}\\
&  variational inf&22.4613$\pm$\tiny{0.014}&33.6538$\pm$\tiny{0.017}&&0.7214$\pm$\tiny{0.029}&0.1907$\pm$\tiny{0.032}&0.1522$\pm$\tiny{0.016}&1.5192$\pm$\tiny{0.021}&0.9455$\pm$\tiny{0.055}&1.5939$\pm$\tiny{0.003}\\
&bio  dnn&24.9822$\pm$\tiny{0.041}&\textbf{51.6026$\pm$\tiny{0.071}}&&0.6764$\pm$\tiny{0.076}&0.2262$\pm$\tiny{0.013}&0.1334$\pm$\tiny{0.031}&1.3928$\pm$\tiny{0.068}&0.6571$\pm$\tiny{0.114}&1.5596$\pm$\tiny{0.011}\\
&bio  dropconnect&\underline{27.0293$\pm$\tiny{0.033}}&47.1154$\pm$\tiny{0.075}&&0.841$\pm$\tiny{0.043}&0.3441$\pm$\tiny{0.053}&0.1738$\pm$\tiny{0.007}&\textbf{1.4297$\pm$\tiny{0.06}}&0.7276$\pm$\tiny{0.118}&\textbf{1.5419$\pm$\tiny{0.02}}\\
&bio  mc dropout&26.8859$\pm$\tiny{0.008}&47.1154$\pm$\tiny{0.019}&&0.6843$\pm$\tiny{0.07}&0.224$\pm$\tiny{0.054}&0.1294$\pm$\tiny{0.036}&1.4363$\pm$\tiny{0.012}&0.9167$\pm$\tiny{0.062}&1.5732$\pm$\tiny{0.009}\\
&bio  variational inf&24.3715$\pm$\tiny{0.041}&41.0256$\pm$\tiny{0.087}&&0.774$\pm$\tiny{0.019}&0.2724$\pm$\tiny{0.058}&0.1672$\pm$\tiny{0.014}&1.4467$\pm$\tiny{0.061}&0.8045$\pm$\tiny{0.024}&1.5601$\pm$\tiny{0.018}\\

\midrule
%=============================================================================
         \parbox[t]{2mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{PXSLU}}} & 
         DNN&32.2541$\pm$\tiny{0.075}&88.2452$\pm$\tiny{0.012}&&0.5743$\pm$\tiny{0.077}&0.4556$\pm$\tiny{0.094}&0.2955$\pm$\tiny{0.014}&1.2807$\pm$\tiny{0.05}&0.995$\pm$\tiny{0.004}&1.3821$\pm$\tiny{0.003}\\
& dropconnect&34.1464$\pm$\tiny{0.026}&84.2989$\pm$\tiny{0.05}&&0.4599$\pm$\tiny{0.088}&0.3936$\pm$\tiny{0.047}&0.2354$\pm$\tiny{0.03}&1.2154$\pm$\tiny{0.062}&\textbf{1.0$\pm$\tiny{0.0}}&1.3768$\pm$\tiny{0.007}\\
& mc dropout&32.4014$\pm$\tiny{0.076}&87.9093$\pm$\tiny{0.015}&&0.5412$\pm$\tiny{0.107}&0.4905$\pm$\tiny{0.092}&0.2667$\pm$\tiny{0.028}&1.2684$\pm$\tiny{0.064}&\textbf{1.0$\pm$\tiny{0.0}}&1.3815$\pm$\tiny{0.004}\\
& variational inf&31.546$\pm$\tiny{0.137}&\underline{90.3442$\pm$\tiny{0.012}}&&0.3913$\pm$\tiny{0.213}&0.374$\pm$\tiny{0.201}&0.1959$\pm$\tiny{0.085}&1.1455$\pm$\tiny{0.185}&0.9966$\pm$\tiny{0.006}&1.3612$\pm$\tiny{0.034}\\
&bio dnn&33.1131$\pm$\tiny{0.097}&80.1763$\pm$\tiny{0.238}&&0.5389$\pm$\tiny{0.116}&0.3929$\pm$\tiny{0.057}&0.2867$\pm$\tiny{0.037}&1.2548$\pm$\tiny{0.06}&0.9831$\pm$\tiny{0.018}&1.38$\pm$\tiny{0.003}\\
&bio dropconnect&\textbf{40.3372$\pm$\tiny{0.07}}&89.1184$\pm$\tiny{0.039}&&0.2649$\pm$\tiny{0.127}&0.2576$\pm$\tiny{0.105}&0.1568$\pm$\tiny{0.058}&1.0539$\pm$\tiny{0.111}&0.9997$\pm$\tiny{0.001}&1.3496$\pm$\tiny{0.021}\\
&bio mc dropout&\underline{37.4772$\pm$\tiny{0.031}}&\textbf{91.2678$\pm$\tiny{0.013}}&&0.5048$\pm$\tiny{0.04}&0.5048$\pm$\tiny{0.019}&0.2609$\pm$\tiny{0.014}&1.2472$\pm$\tiny{0.026}&\textbf{1.0$\pm$\tiny{0.0}}&1.3805$\pm$\tiny{0.002}\\
&bio variational inf&37.3134$\pm$\tiny{0.046}&88.2452$\pm$\tiny{0.057}&&\textbf{0.225$\pm$\tiny{0.111}}&\textbf{0.205$\pm$\tiny{0.089}}&\textbf{0.1255$\pm$\tiny{0.055}}&\textbf{1.0117$\pm$\tiny{0.109}}&0.9992$\pm$\tiny{0.001}&1.34$\pm$\tiny{0.024}\\

\midrule
%=============================================================================
         \parbox[t]{2mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{MEDMCQA}}} & 
         DNN&28.5727$\pm$\tiny{0.03}&\underline{63.88$\pm$\tiny{0.055}}&&0.6787$\pm$\tiny{0.1}&0.3256$\pm$\tiny{0.043}&0.1575$\pm$\tiny{0.021}&1.5347$\pm$\tiny{0.062}&0.9625$\pm$\tiny{0.033}&1.6063$\pm$\tiny{0.003}\\
& dropconnect&\textbf{32.0291$\pm$\tiny{0.003}}&63.5584$\pm$\tiny{0.007}&&\textbf{0.4822$\pm$\tiny{0.015}}&\textbf{0.165$\pm$\tiny{0.01}}&\textbf{0.1099$\pm$\tiny{0.0}}&\textbf{1.3846$\pm$\tiny{0.009}}&0.9764$\pm$\tiny{0.007}&1.5888$\pm$\tiny{0.001}\\
& mc dropout&28.3648$\pm$\tiny{0.029}&61.3612$\pm$\tiny{0.103}&&0.7533$\pm$\tiny{0.044}&0.3819$\pm$\tiny{0.084}&0.1518$\pm$\tiny{0.02}&1.5848$\pm$\tiny{0.024}&\textbf{1.0$\pm$\tiny{0.0}}&1.6091$\pm$\tiny{0.0}\\
& variational inf&23.1977$\pm$\tiny{0.042}&48.5531$\pm$\tiny{0.046}&&0.7499$\pm$\tiny{0.023}&0.242$\pm$\tiny{0.033}&0.1329$\pm$\tiny{0.004}&1.5822$\pm$\tiny{0.013}&\textbf{1.0$\pm$\tiny{0.0}}&1.6089$\pm$\tiny{0.0}\\
&bio dnn&28.1549$\pm$\tiny{0.045}&61.0932$\pm$\tiny{0.089}&&0.6859$\pm$\tiny{0.12}&0.3026$\pm$\tiny{0.009}&0.1582$\pm$\tiny{0.01}&1.5388$\pm$\tiny{0.077}&0.9775$\pm$\tiny{0.02}&1.6064$\pm$\tiny{0.004}\\
&bio dropconnect&29.7558$\pm$\tiny{0.07}&60.343$\pm$\tiny{0.103}&&0.6687$\pm$\tiny{0.17}&0.2973$\pm$\tiny{0.069}&0.1278$\pm$\tiny{0.018}&1.5216$\pm$\tiny{0.122}&0.9893$\pm$\tiny{0.019}&1.6025$\pm$\tiny{0.012}\\
&bio mc dropout&\underline{32.0019$\pm$\tiny{0.013}}&\textbf{70.5788$\pm$\tiny{0.012}}&&0.5655$\pm$\tiny{0.096}&0.3481$\pm$\tiny{0.06}&0.1551$\pm$\tiny{0.025}&1.4663$\pm$\tiny{0.068}&0.9962$\pm$\tiny{0.006}&1.602$\pm$\tiny{0.006}\\
&bio variational inf&27.5691$\pm$\tiny{0.012}&52.3044$\pm$\tiny{0.024}&&0.7294$\pm$\tiny{0.021}&0.2559$\pm$\tiny{0.018}&0.1266$\pm$\tiny{0.004}&1.5701$\pm$\tiny{0.012}&\textbf{1.0$\pm$\tiny{0.0}}&1.6084$\pm$\tiny{0.001}\\

\midrule
%=============================================================================
         \parbox[t]{2mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{MORFITT}}} & 
         DNN&49.7506$\pm$\tiny{0.009}&59.038$\pm$\tiny{0.012}&&0.6499$\pm$\tiny{0.022}&0.2323$\pm$\tiny{0.021}&0.0398$\pm$\tiny{0.005}&2.0748$\pm$\tiny{0.015}&0.796$\pm$\tiny{0.045}&2.4454$\pm$\tiny{0.003}\\
& dropconnect&\underline{55.4551$\pm$\tiny{0.01}}&\underline{62.5306$\pm$\tiny{0.008}}&&0.6134$\pm$\tiny{0.003}&0.2243$\pm$\tiny{0.003}&0.0425$\pm$\tiny{0.001}&2.0332$\pm$\tiny{0.006}&0.8775$\pm$\tiny{0.014}&2.4411$\pm$\tiny{0.001}\\
& mc dropout&51.2184$\pm$\tiny{0.02}&60.386$\pm$\tiny{0.018}&&0.5877$\pm$\tiny{0.009}&0.0934$\pm$\tiny{0.021}&\textbf{0.0308$\pm$\tiny{0.002}}&2.1249$\pm$\tiny{0.028}&0.9427$\pm$\tiny{0.006}&2.4589$\pm$\tiny{0.004}\\
& variational inf&53.6771$\pm$\tiny{0.017}&61.4583$\pm$\tiny{0.025}&&0.6024$\pm$\tiny{0.049}&0.1905$\pm$\tiny{0.074}&0.0392$\pm$\tiny{0.009}&2.0513$\pm$\tiny{0.026}&0.8725$\pm$\tiny{0.06}&2.4452$\pm$\tiny{0.007}\\
 &bio dnn&53.4963$\pm$\tiny{0.019}&61.8015$\pm$\tiny{0.014}&&0.6081$\pm$\tiny{0.017}&0.2098$\pm$\tiny{0.014}&0.0363$\pm$\tiny{0.002}&2.0538$\pm$\tiny{0.015}&0.8334$\pm$\tiny{0.01}&2.4453$\pm$\tiny{0.002}\\
&bio dropconnect&\textbf{56.4418$\pm$\tiny{0.018}}&\textbf{62.9596$\pm$\tiny{0.02}}&&0.6148$\pm$\tiny{0.027}&0.2325$\pm$\tiny{0.018}&0.0433$\pm$\tiny{0.003}&\textbf{2.0251$\pm$\tiny{0.015}}&0.8667$\pm$\tiny{0.03}&\textbf{2.4394$\pm$\tiny{0.001}}\\
&bio mc dropout&52.6114$\pm$\tiny{0.008}&61.2132$\pm$\tiny{0.004}&&0.5942$\pm$\tiny{0.004}&0.1275$\pm$\tiny{0.027}&0.0332$\pm$\tiny{0.003}&2.1046$\pm$\tiny{0.021}&0.9455$\pm$\tiny{0.002}&2.4551$\pm$\tiny{0.003}\\
&bio variational inf&53.2133$\pm$\tiny{0.01}&61.5502$\pm$\tiny{0.006}&&\textbf{0.5449$\pm$\tiny{0.005}}&\textbf{0.0546$\pm$\tiny{0.005}}&0.0324$\pm$\tiny{0.001}&2.1594$\pm$\tiny{0.008}&\textbf{0.9911$\pm$\tiny{0.003}}&2.4675$\pm$\tiny{0.001}\\


         \bottomrule
    \end{tabular}
    }
    \caption{Comparison for text classification performance and uncertainty-awareness. We report the mean of 3 seed runs for all the metrics. We denote best score with \textbf{bold} and second best with \underline{underline}. Here, BNN denotes {DropConnect} as it was on average the best ranked model across all the best configurations.  }
    \label{tab:finalcomparisontable-all-new}
\end{table*}

\begin{comment}
    i have a simple with siunitx i'll paste below, might be easier than what you're doing right now

\sisetup{
separate-uncertainty,
table-align-uncertainty,
table-format = 2.1(1),
detect-weight=true}
\begin{tabular}{p{0.5cm}@{{\,\,}}p{0.75cm}@{{\,\,}}l@{{\,}}l  >{\columncolor{gray!25}}S@{{\quad}}S@{{\quad}}>{\columncolor{gray!25}}S@{{\quad}}S@{{\quad}}>{\columncolor{gray!25}}S@{{\quad}}S }
&& \multicolumn{2}{@{{}}c}{\multirow{2}{*}{\pbox{1.75cm}{\textbf{Translation} \newline \textbf{directions}}}} &&&&& \\ 
&&&& $\mathcal{N}$ & $\mathcal{F}$ & $\mathcal{E}$ & $\mathcal{D}$ & $\mathcal{T}$ & $\mathcal{L}$  \\
\toprule
\multirow{12}{*}{\rotatebox{90}{test on \textbf{UNPC}}}
&\multirow{7}{*}{\rotatebox{90}{train on \textbf{UNPC}}}
& \textbf{All} & (seen) & 26.6(0.5) & \bf 28.2(1.1) &  \uline{$\mathbf{29.0 \pm 0.2}$} & 24.8(0.2) & 26.6(0.1) & 26.4(0.2) \\
\cmidrule(lr){3-10}
&&\multirow{3}{*}{\textbf{AR}} 
& all & 18.1(0.3) &  \uline{$\mathbf{24.6 \pm 1.3}$} & \bf 23.1(1.7) & 15.7(1.8) & 16.8(0.4) & 17.9(0.1) \\
&&& seen & 26.4(0.1) & \uline{$\mathbf{27.1\pm 0.9}$} & \bf 26.6(0.7) & 22.0(1.0) & 24.9(0.1) & {$26.2 \pm 0.0$} \\
&&& unseen & 13.9(0.3) &  \uline{$\mathbf{23.4\pm 1.4}$} & \bf 21.4(2.3) & 12.5(2.2) & 12.8(0.6) & 13.7(0.1) \\
\cmidrule(lr){3-10}
&&\multirow{3}{*}{\textbf{EN}} 
& all & 19.3(0.4) & \bf 22.8(2.9) &  \uline{$\mathbf{23.9\pm 1.0}$} & 17.9(0.4) & 19.3(0.1) & 19.4(0.1) \\
&&& seen & 34.5(0.2) & 33.1(2.6) &  \uline{$\mathbf{35.9\pm 0.1}$} & 31.6(0.9) & 34.0(0.2) & \bf 34.6(0.3) \\
&&& unseen & 11.7(00.6) &  \bf 17.6(3.0) &  \uline{$\mathbf{17.9\pm 1.4}$} & 11.0(1.0) & 11.9(0.1) & 11.8(0.1) \\
\cmidrule{2-10}
&\multirow{3}{*}{\rotatebox{90}{\pbox{1.75cm}{train on \\ \textbf{OPUS}}}}
&\multirow{3}{*}{\textbf{EN}}
& all & 16.4(0.2) & \bf 20.6(0.5) &  \uline{$\mathbf{20.9 \pm 0.4}$} & 13.6(1.2) & 16.8(0.2) & 16.3(0.1) \\
&&& seen  & \bf 30.8(0.2) & 30.5(0.5) &  \uline{$\mathbf{31.1 \pm 0.3}$} & 23.7(1.5) & 30.7(0.3) & 30.6(0.3) \\
&&& unseen & 9.1(0.3) & \bf 15.6(0.5) &  \uline{$\mathbf{15.8 \pm 0.5}$} & 8.5(1.0) & 9.9(0.1) & 9.1(0.1) \\


\midrule
\multirow{12}{*}{\rotatebox{90}{test on \textbf{OPUS}}}
&\multirow{7}{*}{\rotatebox{90}{train on \textbf{UNPC}}}
& \textbf{All} & (seen) & 17.6(0.2) & \bf 19.1(0.8) & \uline{$\mathbf{19.7 \pm 0.2}$} & 16.3(0.2) & 17.5(0.2) & 17.5(0.3) \\
\cmidrule(lr){3-10}
&&\multirow{3}{*}{\textbf{AR}} 
& all & 12.3(0.2) & \uline{$\mathbf{16.5 \pm 0.8}$} & \bf 15.4(1.0) & 10.3(1.4) & 11.4(0.2) & 12.1(0.1) \\
&&& seen & 17.7(0.1) & \uline{$\mathbf{18.4 \pm 0.8}$} & \bf 17.9(0.6) & 13.8(1.0) & 16.6(0.1) & 17.6(0.1)  \\
&&& unseen  & 9.2(0.3) & \uline{$\mathbf{15.5 \pm 0.8}$} & \bf 13.9(1.3) & 8.4(1.6) & 8.5(0.2) & 9.0(0.1) \\
\cmidrule(lr){3-10}
&&\multirow{3}{*}{\textbf{EN}} 
& all & 13.4(0.3) & \bf 15.9(2.0) & \uline{$\mathbf{17.0 \pm 0.5}$} & 12.6(0.2) & 13.3(0.1) & 13.5(0.2) \\
&&& seen  & 19.7(0.1) & \bf 19.8(1.4) & \uline{$\mathbf{21.0 \pm 0.0}$} & 18.5(0.7) & 19.2(0.1) & \bf 19.8(0.2) \\
&&& unseen & 8.2(0.3) & \bf 12.7(2.5) & \uline{$\mathbf{13.6 \pm 0.9}$} & 7.7(0.7) & 8.4(0.3) & 8.2(0.3)  \\
\cmidrule{2-10}
&\multirow{3}{*}{\rotatebox{90}{\pbox{1.75cm}{train on \\ \textbf{OPUS}}}}
&\multirow{3}{*}{\textbf{EN}}
& all  & 15.0(0.2) & \bf 17.8(0.3) & \uline{$\mathbf{17.9 \pm 0.3}$} & 12.4(1.0) & 15.5(0.2) & 14.8(0.1) \\
&&& seen  & \uline{$\mathbf{25.1 \pm 0.2}$} & 24.6(0.3) & \uline{$\mathbf{25.1 \pm 0.2}$} & 19.7(1.6) & 24.9(0.2) & 24.9(0.3)  \\
&&& unseen & 6.6(0.2) & \uline{$\mathbf{12.1 \pm 0.3}$} & \bf 11.8(0.5) & 6.3(0.7) & 7.7(0.2) & 6.4(0.1) \\
\bottomrule
\end{tabular}
\end{comment}

==> Tables/unctcomparison.tex <==
\begin{table*}[]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|cccccc|c}
        \toprule
        %\cellcolor{red!25}
        %\cellcolor{green!25}
        dataset-config & BRIER($\downarrow$) &	ECE($\downarrow$)& 	SCE($\downarrow$) &	NLL($\downarrow$) &	COV\%($\uparrow$) & ENTROPY($\downarrow$) & Win($\mathbb{U}$)\\
        \midrule
        biocamembert 	dnn 	PXCORPUS 	1e-5 	15 &	0.479364 &	0.415783 &	0.274239 	&1.221917 &	\cellcolor{red!25}0.973132&1.378235 \\
        biocamembert 	dropconnect 	PXCORPUS 	1e-5 	15& 	0.227683 &	0.159425 &	0.137527 &	1.001403 &	\cellcolor{red!25}0.962217* &1.335407\\
        biocamembert 	mcdropout 	PXCORPUS 	1e-5 	14& 	0.477025 &	0.422855* &	0.267388 &	1.219310& 	\cellcolor{red!25}0.992443 &1.377620\\
        biocamembert 	variationalinf 	PXCORPUS 	1e-5 	12& 	0.210911 &	0.158169& 	0.115819 &	0.989729 &	\cellcolor{red!25}0.970613* &1.333781\\       
        \hdashline
        camembert 	dnn 	PXCORPUS 	1e-5 	14& 	0.533842 &	0.467537 &	0.276416 &	1.261665 &	0.997481&1.380891\\
        camembert 	dropconnect 	PXCORPUS 	5e-6 	14&  0.365078 &	0.316629 &	0.212358 	&1.145101& 	0.962217*&1.368281\\
        camembert 	mcdropout 	PXCORPUS 	1e-5 	14& 0.518185 	&0.432743 	&0.272942 &	1.248371 &	0.994962*	&1.379459 	\\
        camembert 	variationalinf 	PXCORPUS 	1e-5 	10&  0.378961 &	0.335311 	&0.190471 &	1.126968 &	0.977330*&1.356247\\
        \midrule
        %===========================================================
        biocamembert 	dnn 	MEDMCQA 	5e-6 	15& 	0.696034 	&\cellcolor{red!25}0.354713 &	0.152432 &	1.546633 	&\cellcolor{red!25}0.981243&1.607683\\
        biocamembert 	dropconnect 	MEDMCQA 	5e-6 	14&  0.673225 	&0.274169& 	0.152654* &	1.524824 &	\cellcolor{red!25}0.987138&1.603390\\
        biocamembert 	mcdropout 	MEDMCQA 	1e-5 	14 & 0.532169 &	0.259087 &	0.148577 &	1.429045& 	\cellcolor{red!25}0.961951*&1.596767\\        
        biocamembert 	variationalinf 	MEDMCQA 	1e-6 	15& 	0.732524* &	0.156790 &	\cellcolor{red!25}0.135397 &	1.564276* &	0.924437*&1.607780*\\
        \hdashline
        camembert 	dnn 	MEDMCQA 	5e-6 	11 	&	0.725581 	&0.352222 &	0.171180 &	1.566691& 	0.983387&1.608586\\
        camembert 	dropconnect 	MEDMCQA 	1e-6 	15& 	0.725009 &	0.303931 &	0.157625 &	1.567476* 	&0.988210&1.608650*\\
        camembert 	mcdropout 	MEDMCQA 	5e-6 	11 &	0.749677 &	0.347507 &	0.165071 &	1.580934* &	0.989818&1.608975*\\
        camembert 	variationalinf 	MEDMCQA 	1e-6 	15& 	0.746021 &	0.231534 &	0.126477 	&1.579299* 	&0.825295* &1.608702*\\
        \midrule
        %===========================================================
        biobert 	dnn 	SMOKING 	1e-4 	15 	&	\cellcolor{red!25}0.802114 &	\cellcolor{red!25}0.340216 &	\cellcolor{red!25}0.161939 &	1.421092 &	0.682692&1.546859\\
        biobert 	dropconnect 	SMOKING 	5e-5 	13 &	\cellcolor{red!25}0.763660 &	\cellcolor{red!25}0.273658 &	\cellcolor{red!25}0.154944 	&1.411110 &	\cellcolor{red!25}0.541667*&1.551109*\\
        biobert 	mcdropout 	SMOKING 	5e-5 	13& 	0.693898 &	0.203049 &	\cellcolor{red!25}0.129748 	&\cellcolor{red!25}1.431387* &	0.669872*&\cellcolor{red!25}1.570405*\\
        biobert 	variationalinf 	SMOKING 	5e-5 	13& 	\cellcolor{red!25}0.807533* 	&\cellcolor{red!25}0.291873& 	0.162787* &	1.453634* 	&\cellcolor{red!25}0.532051*&1.558958*\\
        \hdashline
        bert 	dnn 	SMOKING 	5e-5 	9 &	0.669931 &	0.170088 &	0.132612 &	1.473753 &	0.612179&1.588659\\
        bert 	dropconnect 	SMOKING 	1e-5 	14 &	0.620675 &	0.127112 &	0.109565 &	1.421468 &	0.647436&1.578952\\
        bert 	mcdropout 	SMOKING 	5e-5 	14 &0.709014* &	0.239418* &	0.127739 &	1.417560 &	0.650641&1.562410\\
        bert 	variationalinf 	SMOKING 	5e-6 	10 &	0.748128* &	0.197313* &	0.165275* &	1.495207*& 	0.567308*&1.584503\\
        \midrule
        %===========================================================
        biobert 	dnn 	MEDABS 	5e-5 	5& \cellcolor{red!25}0.571310 &	\cellcolor{red!25}0.180296 &	\cellcolor{red!25}0.077107 &	1.310785 &	0.912512	&1.548926\\
        biobert 	dropconnect 	MEDABS 	5e-5 	3 &0.523878& 	0.140859 &	0.062842 &	1.291286 &	0.856994*&1.550856*\\
        biobert 	mcdropout 	MEDABS 	1e-4 	3 	&	0.535788 &	0.109194 &	0.063076 &	1.321559* &	\cellcolor{red!25}0.899469*&\cellcolor{red!25}1.559733*\\
        biobert 	variationalinf 	MEDABS 	1e-4 	4 &	0.546861 	&\cellcolor{red!25}0.158790 &\cellcolor{red!25}	0.070237 &	1.295509 &	0.802516*&1.548432\\
        
        \hdashline
        bert 	dnn 	MEDABS 	5e-6 	6 	&0.551441 &	0.134095 &	0.066295 &	1.331350 &	0.896353&1.560235\\
        bert 	dropconnect 	MEDABS 	1e-6 	15 &	0.557037* &	0.145812* &	0.069479* &	1.325999 &	0.855494*&1.557213\\
        bert 	mcdropout 	MEDABS 	5e-5 	3 &	0.556467* &	0.137869* &	0.065991 &	1.325434 &	0.901777&1.557578\\
        bert 	variationalinf 	MEDABS 	1e-5 	4 &	0.559371* &	0.134518* &	0.068471* &	1.321513 &	0.792590*&1.556110\\
        \midrule
        %===========================================================
        
        
        biocamembert 	dnn 	MORFITT 	5e-5 	15 &	\cellcolor{red!25}0.597271 	&\cellcolor{red!25}0.195975 &	0.034757 	&2.055853 	&\cellcolor{red!25}0.837929& 2.446618\\
        biocamembert 	dropconnect 	MORFITT 	5e-5 	11& \cellcolor{red!25}0.623643* &	\cellcolor{red!25}0.254945* &	\cellcolor{red!25}0.043031* &	2.015742& 	\cellcolor{red!25}0.754289*&2.436898\\
        biocamembert 	mcdropout 	MORFITT 	5e-5 	15 &	\cellcolor{red!25}0.618586* &	\cellcolor{red!25}0.201053* &	\cellcolor{red!25}0.037850* &	2.069163* 	&\cellcolor{red!25}0.823223*&2.447151*\\
        biocamembert 	variationalinf 	MORFITT 	1e-5 	14& 0.553047 &	0.066514 &	0.032891& \cellcolor{red!25}	2.123252* &	0.827206*&\cellcolor{red!25}2.461358\\
        
        
        camembert 	dnn 	MORFITT 	5e-5 	11& 		0.591286 &	0.060664 &	0.039075& 	2.171540 &	0.877757&2.466179\\
        camembert 	dropconnect 	MORFITT 	5e-5 	6 &	0.587825 &	0.073795* &	0.040320* &	2.180531* &	0.883272&2.467595*\\
        camembert 	mcdropout 	MORFITT 	5e-5 	14& 	0.605074* &	0.168064* &	0.034935 &	2.088549 &	0.834559*&2.451635\\
        camembert 	variationalinf 	MORFITT 	5e-5 	10& 	0.628891* 	&0.237061* &	0.042748* 	&2.029523 &	0.733150*&2.439201\\
        \midrule
        %===========================================================
        biobert 	dnn 	MEDNLI 	1e-5 	12& 		 	0.360875 	&0.147122 	&0.099788& 	0.766016 	&0.863338& 	0.995832\\
biobert dropconnect 	MEDNLI 	5e-6 	11& 	  	0.313292 &	0.120978 &	0.082146 	&0.744658 &	0.877637 &	0.997812\\
biobert mcdropout 	MEDNLI 	1e-5 	15& 	  	0.341800& 	0.148329 &	0.098553 &	0.747583 &	0.857947 	&0.990527 \\
biobert variationalinf 	MEDNLI 	5e-6 	13&  	0.366246 &	0.110367 	&0.078582 &	0.797119 &	0.882560 &	1.013314\\
        \hdashline
        bert 	dnn 	MEDNLI 	5e-6 	10 &	0.402373& 	0.115560 &	0.077374 &	0.828362 &	0.928504 	&1.020356\\
bert dropconnect 	MEDNLI 	1e-5 	15& 	  	0.435817 &	0.202691& 	0.136461& 	0.790006 &	0.807079 &	0.988143 \\
bert mcdropout 	MEDNLI 	1e-5 	8 &		0.411019 &	0.134725 &	0.089256 &	0.823002& 	0.890764 	&1.015102 \\
bert variationalinf 	MEDNLI 	1e-5 	14& 	 	0.451725 &	0.187583 &	0.127065 &	0.819217 &	0.816221 	&1.001283 \\

        %===========================================================
        %\rowcolor{gray!45}
        %& val-mae 	&test-mae &	val-rmse &	test-rmse \\
        %biobert 	dnn regressor 	BIOSSES 	5e-4 	12& 	0.900200 	&1.184433& 	1.114300 	&1.387067 \\
        %biobert 	vi regressor 	BIOSSES 	5e-4 	16 &	1.191400 &	1.161567 &	1.420900 	&1.419900 \\
        %biobert 	mcd regressor 	BIOSSES 	1e-5 	13 &	0.879900 &	1.191433 &	1.088433 &	1.402167\\
        %biobert 	dc regressor 	BIOSSES 	1e-6 	98 &	1.412633 	&1.627133 &	1.650567 &	1.931433 \\
        %\hdashline
        %bert 	mcd regressor 	BIOSSES 	5e-4 	4 	&0.792567 &	1.146767 	&1.034533 &	1.318533 \\
        %bert 	dc regressor 	BIOSSES 	1e-6 	84& 	1.132667 &	1.375867 &	1.356667 	&1.620067 \\
        %bert 	vi regressor 	BIOSSES 	5e-6 	21 &	1.240867 &	1.279133 &	1.523233 &	1.484567 \\
        %bert 	dnn regressor 	BIOSSES 	5e-4 	11 &	1.084600 &	1.385167 &	1.331533 &	1.619300 \\
        
         %& \\
         \bottomrule
    \end{tabular}}
    \caption{New Uncertainty Table on test set, * denotes unexpected score compared to DNN counterpart}
    \label{tab:newperf}
\end{table*}
